Wavelet entropy and fractional Brownian motion time series

We study the functional link between the Hurst parameter and the Normalized Total Wavelet Entropy when analyzing fractional Brownian motion (fBm) time series--these series are synthetically generated. Both quantifiers are mainly used to identify fractional Brownian motion processes (Fractals 12 (2004) 223). The aim of this work is understand the differences in the information obtained from them, if any.

==> pstricks-add.tex <==
%%
%% This is file `pstricks-add.tex',
%%
%% IMPORTANT NOTICE:
%%
%% Package `pstricks-add.tex'
%%
%% Herbert Voss <voss@perce.de>
%%
%% This program can be redistributed and/or modified under the terms
%% of the LaTeX Project Public License Distributed from CTAN archives
%% in directory macros/latex/base/lppl.txt.
%%
%% DESCRIPTION:
%%   `pstricks-add' is a PSTricks package for additionals to the standard
%%         pstricks package
%%
\def\fileversion{0.9b}
\let\pstricksAddFV\fileversion
\def\filedate{2003/11/15}
\message{`pstricks-add' v\fileversion, \filedate\space (Herbert Voss)}
\csname PSTricksAddLoaded\endcsname
\let\PSTricksAddLoaded\endinput
% Requires PSTricks, pst-node
\usepackage{pstcol}
\ifx\PSTricksLoaded\endinput\else\input pstricks \fi
\ifx\PSTnodesLoaded\endinput\else\input pst-node \fi
\usepackage{multido}
%
\input pst-key
%
\edef\PstAtCode{\the\catcode`\@} \catcode`\@=11\relax
\SpecialCoor
%
\define@key{psset}{intSeparator}{\edef\psk@intSeparator{#1}}
\setkeys{psset}{intSeparator=\,}
%
\def\psFormatInt{\@ifnextchar[{\psFormatInt@i}{\psFormatInt@i[]}}
\def\psFormatInt@i[#1]#2{{%
	\def\ps@tempa{#1}
	\ifx\ps@tempa\@empty\else\psset{#1}\fi
	\count1=#2\count2=\count1
	\ifnum\count1=0 0\else
		\ifnum\count1>999999
			\count3=\count1
			\divide\count3 by 1000000
			\the\count3\psk@intSeparator
			\multiply\count3 by 1000000
			\advance\count1 by -\count3 % modulo 1000000
		\fi
		\ifnum\count2>999
			\count3=\count1
			\divide\count3 by 1000
			\ifnum\count2>99999
				\ifnum\count3<100 0\fi
				\ifnum\count3<10 0\fi
			\fi
			\the\count3\psk@intSeparator
			\multiply\count3 by 1000
			\advance\count1 by -\count3 %modulo 1000
		\fi%
		\ifnum\count2>999
			\ifnum\count1<100 0\fi
			\ifnum\count1<10 0\fi
		\fi
		\the\count1
	\fi
}}
%
% a new fillstyle
\def\psfs@asolid{\pst@fill{\pst@usecolor\psfillcolor eofill}}
%
\define@key{psset}{braceWidth}{\edef\psk@braceWidth{#1}}
\define@key{psset}{bracePos}{\edef\psk@bracePos{#1}}
\setkeys{psset}{braceWidth=0.35,bracePos=0.5}
%
\def\@@rput@iv(#1){\pst@killglue\pst@makebox{\@@rput@v{#1}}}
\def\@@rput@v#1{%
	\begingroup
		\use@par
		\pst@makesmall\pst@hbox
		\pst@Verb{%
			Alpha 90 sub \psk@braceWidth\space 0 lt {180 add} if
			\ifx\psk@rot\@empty\else\psk@rot add \fi
			/rotAngle exch def
		}%
		\setbox\pst@hbox=\hbox{%
			\pst@Verb{rotAngle \tx@RotBegin}%
			\box\pst@hbox\pst@Verb{\tx@RotEnd}%
		}%
		\psput@{#1}\pst@hbox
	\endgroup
	\ignorespaces%
}
%
\def\psbrace{\@ifnextchar[{\@psbrace}{\@psbrace[]}}
\def\@psbrace[#1](#2)(#3)#4{{
	\setkeys{psset}{linearc=0.2,linewidth=1pt,%
		nodesepA=0pt,nodesepB=0pt,bracePos=0.5}% the default
	\setkeys{psset}{#1}%
	\pst@getcoor{#2}\pst@tempa%
	\pst@getcoor{#3}\pst@tempb%
	\pnode(!%
		/bW2 \psk@braceWidth\space 2.0 div def
		\pst@tempa /YA exch \pst@number\psyunit div def
		/XA exch \pst@number\psxunit div def
		\pst@tempb /YB exch \pst@number\psyunit div def
		/XB exch \pst@number\psxunit div def
		/Alpha YB YA sub XB XA sub atan def
		/xMid XB XA sub \psk@bracePos\space mul XA add def
		/yMid YB YA sub \psk@bracePos\space mul YA add def
		/@deltaX Alpha sin bW2 mul def
		/@deltaY Alpha cos bW2 mul def
		/@xTemp xMid @deltaX 2 mul add def
		/@yTemp yMid @deltaY 2 mul sub def
		@xTemp @yTemp){@tempNode}
	\pst@getcoor{@tempNode}\pst@tempc%
	\@@rput@iv(! %
		\pst@tempc /Yc exch def
		/Xc exch def
		Xc \psk@nodesepA\space add \pst@number\psxunit div
		Yc \psk@nodesepB\space add \pst@number\psxunit div ){#4}
	\psline(#2)%
		(! XA @deltaX add YA @deltaY sub)%
		(! @xTemp @deltaX sub @yTemp @deltaY add)%
		(@tempNode)
	\psline(@tempNode)%
		(! @xTemp @deltaX sub @yTemp @deltaY add)%
		(! XB @deltaX add YB @deltaY sub)%
		(#3)%
}}
%
% from Dennis Giroux: http://www.tug.org/pipermail/pstricks/2001/000507.html
%
% I - Definition of \PstWedgeEllipse, a generalization of \pswedge for wedges
%     of ellipses (from the code of \pswedge and \psellipse)
%
\def\psWedgeEllipse{\def\pst@par{}\pst@object{psWedgeEllipse}}
\def\psWedgeEllipse@i(#1){%
	\@ifnextchar({\psWedgeEllipse@ii(#1)}{\pstWedgeEllipse@ii(0,0)(#1)}}
\def\psWedgeEllipse@ii(#1)(#2)#3#4{%
	\begin@ClosedObj
		\pst@getangle{#3}\pst@tempa
		\pst@getangle{#4}\pst@tempb
		\pst@getcoor{#1}\pst@tempc
		\pst@@getcoor{#2}%
		\def\pst@linetype{1}%
		\addto@pscode{%
			\pst@tempa \pst@tempb
			\pst@coor
			\pst@tempc moveto
			\ifdim\psk@dimen\p@=\z@\else
				\psk@dimen CLW mul dup 3 1 roll
				sub 3 1 roll sub exch
			\fi
			\pst@tempc
			\tx@Ellipse
			closepath%
		}%
		\showpointsfalse
	\end@ClosedObj%
}
%
% arcs
%
\def\psEllipticArcN{\def\pst@par{}\pst@object{psellipticarcn}}
\def\psellipticarcn@i{\let\if@psarcn\iftrue\psellipticarc@ii}
%
\def\psEllipticArc{\def\pst@par{}\pst@object{psellipticarc}}
\def\psellipticarc@i{\let\if@psarcn\iffalse\psellipticarc@ii}
%
\let\if@psarcn\iffalse
\def\psellipticarc@ii{\pst@getarrows\psellipticarc@iii}
\def\psellipticarc@iii(#1){%
	\@ifnextchar({\psellipticarc@iv(#1)}{\psellipticarc@iv(0,0)(#1)}}
\def\psellipticarc@iv(#1)(#2)#3#4{%
	\begin@OpenObj
		\pst@getcoor{#1}\pst@tempa
		\pst@getcoor{#2}\pst@tempb
		\pst@getangle{#3}\pst@tempc
		\pst@getangle{#4}\pst@tempd
		\addto@pscode{\psellipticarc@definearg \psellipticarc@draw}%
		\showpointsfalse
	\end@OpenObj%
}
\def\psellipticarc@definearg{%
	\pst@tempa /y ED /x ED  % Origin
	\pst@tempb              % radii. Now adjust:
	\ifdim\psk@dimen\p@=\z@\else
		\psk@dimen CLW mul dup 3 1 roll
		sub 3 1 roll sub exch
	\fi
	/ry ED /rx ED
	/angleA
		/d  {  \if@psarcn sub \else add \fi } def
		\pst@tempc \psk@arcsepA 2 div
		\tx@ArcAdjust
	def
	/angleB
		/d  {  \if@psarcn add \else sub \fi } def
		\pst@tempd \psk@arcsepB 2 div
		\tx@ArcAdjust
	def
	\ifshowpoints\psellipticarc@showpoints\fi
	\ifx\psk@arrowA\@empty
		\ifnum\psk@liftpen=2
			angleA cos rx mul x add
			angleA sin ry mul y add
			moveto
		\fi
	\fi%
}
\def\psellipticarc@draw{%
	0 0 1
	angleA
	\ifx\psk@arrowA\@empty\else
		{ ArrowA CP }
		{ \if@psarcn sub \else add \fi }
		\tx@EllipticArcArrow
	\fi
	angleB
	\ifx\psk@arrowB\@empty\else
		{ ArrowB }
		{ \if@psarcn add \else sub \fi }
		\tx@EllipticArcArrow
	\fi
	/mtrx CM def
	x y T
	rx ry scale
	\if@psarcn arcn \else arc \fi
	mtrx setmatrix%
}
\def\psellipticarc@showpoints{%
	gsave
	/mtrx CM def
	x y T
	rx ry scale
	0 0 moveto
	0 0 1 \pst@tempc \pst@tempd
	\ifcase\psarc@type arc \or arcn \fi
	closepath
	mtrx setmatrix
	CLW 2 div SLW
	[ \psk@dash\space ] 0 setdash stroke
	grestore %
}
\pst@def{ArcAdjust}<%
% given a target length (targetLength) and an initial angle (angle0) [in the stack],
% let  M(angle0)=(rx*cos(angle0),ry*sin(angle0))=(x0,y0).
% This computes an angle t such that (x0,y0) is at distance targetLength from the point M(t)=(rx*cos(t),ry*sin(t)).
% NOTE: this an absolute angle, it does not have to be added or substracted to angle0
% contrary to TvZ's code.
% To achieve, this, one iterates the following process: start with some angle t,
% compute the point M' at distance targetLength of (x0,y0) on the semi-line [(x0,y0) M(t)].
% Now take t' (= new angle) so that (0,0) M(t') and M' are aligned.
%
% Another difference with TvZ's code is that we need d (=add/sub) to be defined.
% the value of d = add/sub is used to know on which side we have to move.
% It is only used in the initialisation of the angle before the iteration.
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Input stack:  1: target length 2: initial angle
% variables used : rx, ry, d (=add/sub)
%
	/targetLength ED /angle0 ED
	/x0 rx angle0 cos mul def
	/y0 ry angle0 sin mul def
% we are looking for an angle t such that (x0,y0) is at distance targetLength from the point M(t)=(rx*cos(t),ry*sin(t)))
%initialisation of angle (using 1st order approx = TvZ's code)
	targetLength 57.2958 mul
	angle0 sin rx mul dup mul
	angle0 cos ry mul dup mul
	add sqrt div
% if initialisation angle is two large (more than 90 degrees) set it to 90 degrees
% (if the ellipse is very curved at the point where we draw the arrow, the value can be much more than 360 degrees !)
% this should avoid going on the wrong side (more than 180 degrees) or go near
% a bad attractive point (at 180 degrees)
	dup 90 ge { pop 90 } if
	angle0 exch d
% maximum number of times to iterate the iterative procedure:
	30
% iterative procedure: takes an angle t on top of stack, computes a better angle (an put it on top of stack)
	{ dup
% compute distance D between (x0,y0) and M(t)
	dup cos rx mul x0 sub dup mul exch sin ry mul y0 sub dup mul add sqrt
% if D almost equals targetLength, we stop
	dup targetLength sub abs 1e-5 le { pop exit } if
% stack now contains D t
% compute the point M(t') at distance targetLength of (x0,y0) on the semi-line [(x0,y0) M(t)]:
% M(t')= ( (x(t)-x0)*targetLength/d+x0 , (y(t)-y0)*targetLength/d+y0 )
	exch dup cos rx mul x0 sub  exch sin ry mul y0 sub
% stack contains:  y(t)-y0, x(t)-x0, d
	2 index \tx@Div targetLength mul y0 add ry \tx@Div exch
	2 index \tx@Div targetLength mul x0 add rx \tx@Div
% stack contains x(t')/rx , y(t')/ry , d
% now compute t', and remove D from stack
	atan exch pop
	} repeat
% we don't look at what happened... in particular, if targetLength is greater than the diameter of the ellipse...
% the final angle will be around /angle0 + 180. maybe we should treat this pathological case...
%after iteration, stack contains an angle t such that M(t) is the tail of the arrow
% to give back the result as a an angle relative to angle0 we could add the following line:
% angle0 sub 0 exch d
>
\pst@def{EllipticArcArrow}<%
	/d ED      % add/sub
	/b ED      % arrow procedure
	/a1 ED     % angle
	gsave
	newpath
	0 -1000 moveto
	clip                  % Set clippath far from arrow.
	newpath
	0 1 0 0 b             % Draw arrow to determine length.
	grestore
% Length of arrow is on top of stack. Next 3 numbers are junk.
%
	a1 exch \tx@ArcAdjust   % Angular position of base of arrow.
	/a2 ED
	pop pop pop
	a2 cos rx mul x add
	a2 sin ry mul y add
	a1 cos rx mul x add
	a1 sin ry mul y add
	% Now arrow tip coor and base coor are on stack.
	b pop pop pop pop       % Draw arrow, and discard coordinates.
	a2 CLW 8 div
% change value of d (test it by looking if  `` 1 1 d '' gives 2 or not )
	1 1 d 2 eq { /d { sub } def } { /d { add } def } ifelse
	\tx@ArcAdjust
% resets original value of d
	1 1 d 2 eq { /d { sub } def } { /d { add } def } ifelse>  % Adjust angle to give overlap.
%

%
% -------------- the arrow part -------------
%  the original table
% \def\pst@arrowtable{,<->,<<->>,>-<,>>-<<,(-),[-]}
\edef\pst@arrowtable{\pst@arrowtable,)-(,]-[,|>-<|}
%
\@namedef{psas@<|}{%
    \psk@tbarsize \tx@Tbar
    0 CLW 2 div T
    newpath
    true \psk@arrowinset \psk@arrowlength \psk@arrowsize \tx@Arrow%
}
% ]-[ arrow
\def\tx@BracketOut{BracketOut }
\@namedef{psas@[}{%
	/BracketOut {%
	CLW mul add dup CLW sub 2 div
%/x ED mul CLW add
	/x ED mul neg
	/y ED
	/z CLW 2 div def
	x neg y moveto
	x neg CLW 2 div L x CLW 2 div L x y L stroke 0 CLW moveto } def
	\psk@bracketlength \psk@tbarsize \tx@BracketOut
}
% )-( arrow
\def\tx@RoundBracketOut{RoundBracketOut }
\@namedef{psas@(}{%
	/RoundBracketOut {%
	CLW mul add dup 2 div
%/x ED mul
	/x ED mul neg
	/y ED
	/mtrx CM def
	0 CLW
	2 div T x y mul 0 ne { x y scale } if
	1 1 moveto
	.85 .5 .35 0 0 0 curveto
	-.35 0 -.85 .5 -1 1 curveto
	mtrx setmatrix stroke 0 CLW moveto } def
	\psk@rbracketlength \psk@tbarsize \tx@RoundBracketOut
}
%
% Redefininition of \psset@arrowscale to store value of X scale factor
\def\psset@arrowscale#1{\pst@getscale{#1}\psk@arrowscale}
\psset@arrowscale{1}

\def\psset@arrowscale#1{%
	\psset@arrowscale@i#1 \@nil
	\pst@getscale{#1}\psk@arrowscale%
}
\def\psset@arrowscale@i#1 #2\@nil{\edef\pst@arrowscale{#1}}
\def\pst@arrowscale{1}

% New parameter "arrowfill", with default as "true"
\newif\ifpsArrowFill
\def\psset@ArrowFill#1{\@nameuse{psArrowFill#1}}
\psset@ArrowFill{true}

% Modification of the PostScript macro Arrow to choose to fill or not the arrow
% (it require to restore the current linewidth, despite of the scaling)
\pst@def{Arrow}<{%
    CLW mul add dup 2 div
    /w ED mul dup
    /h ED mul
    /a ED { 0 h T 1 -1 scale } if
    gsave
    \ifpsArrowFill\else
	\pst@number\pslinewidth \pst@arrowscale\space div SLW
    \fi
    w neg h moveto
    0 0 L w h L w neg a neg rlineto
    \ifpsArrowFill gsave fill grestore \else gsave closepath stroke grestore \fi
	grestore
	0 h a sub moveto
}>
\@namedef{psas@>>}{%
    false \psk@arrowinset \psk@arrowlength \psk@arrowsize \tx@Arrow
    0 h a sub T
    gsave
    newpath
    false \psk@arrowinset \psk@arrowlength \psk@arrowsize \tx@Arrow
    CP
    grestore
    moveto
}
%
\@namedef{psas@<<}{%
    true \psk@arrowinset \psk@arrowlength \psk@arrowsize \tx@Arrow
    0 h neg a add T
    false \psk@arrowinset \psk@arrowlength \psk@arrowsize \tx@Arrow
    0 h a 5 mul 2 div sub moveto
}
%
% DG addition begin - Dec. 18/19, 1997 and Oct. 11, 2002
% Adapted from \psset@arrows
\def\psset@ArrowInside#1{%
    \begingroup
		\pst@activearrows
		\xdef\pst@tempg{<#1}%
    \endgroup
    \expandafter\psset@@ArrowInside\pst@tempg\@empty-\@empty\@nil
    \if@pst\else
		\@pstrickserr{Bad intermediate arrow specification: #1}\@ehpa
    \fi%
}
% Adapted from \psset@@arrows
\def\psset@@ArrowInside#1-#2\@empty#3\@nil{%
    \@psttrue
    \def\next##1,#1-##2,##3\@nil{\def\pst@tempg{##2}}%
    \expandafter\next\pst@arrowtable,#1-#1,\@nil
    \@ifundefined{psas@#2}%
		{\@pstfalse\def\psk@ArrowInside{}}%
		{\def\psk@ArrowInside{#2}}%
}
% Default value empty
\def\psk@ArrowInside{}
% Modified version of \pst@addarrowdef
\def\pst@addarrowdef{%
    \addto@pscode{%
		/ArrowA {
			\ifx\psk@arrowA\@empty
				\pst@oplineto
			\else
				\pst@arrowdef{A}
				moveto
			\fi
		} def
		/ArrowB {
			\ifx\psk@arrowB\@empty \else \pst@arrowdef{B} \fi
		} def
% DG addition
		/ArrowInside {
			\ifx\psk@ArrowInside\@empty \else \pst@arrowdefA{Inside} \fi
		} def
	}%
}
% Adapted from \pst@arrowdef
\def\pst@arrowdefA#1{%
	\ifnum\pst@repeatarrowsflag>\z@
		/Arrow#1c [ 6 2 roll ] cvx def Arrow#1c
	\fi
	\tx@BeginArrow
	\psk@arrowscale
	\@nameuse{psas@\@nameuse{psk@Arrow#1}}
	\tx@EndArrow%
}
% ArrowInsidePos parameter (default value 0.5)
\def\psset@ArrowInsidePos#1{\pst@checknum{#1}\psk@ArrowInsidePos}%
\psset@ArrowInsidePos{0.5}
%
% Modified version of \begin@ClosedObj
\def\begin@ClosedObj{%
    \leavevmode
    \pst@killglue
    \begingroup
	\use@par
	\solid@star
	\ifpsdoubleline \pst@setdoublesep \fi
	\pst@addarrowdef% DG addition
	\init@pscode
}
%
% Redefinition of the PostScript /Line macro to print the intermediate
% arrow on each segment of the line
%
\def\psset@ArrowInsideNo#1{\pst@checknum{#1}\psk@ArrowInsideNo}% hv 20031001
\def\psset@ArrowInsideOffset#1{\pst@checknum{#1}\psk@ArrowInsideOffset}% hv 20031001
\psset{ArrowInsideNo=1,ArrowInsideOffset=0}
%
\pst@def{Line}<{%
	NArray n 0 eq not { n 1 eq { 0 0 /n 2 def } if
    (\psk@ArrowInside) length 0 gt {
		2 copy /y1 ED /x1 ED ArrowA x1 y1
    	/n n 1 sub def
    	n {
			4 copy
			/y1 ED /x1 ED /y2 ED /x2 ED
			x1 y1
			\psk@ArrowInsidePos\space 1 gt{
				/Alpha y2 y1 sub x2 x1 sub atan def
				/ArrowPos \psk@ArrowInsideOffset\space def
				/Length x2 x1 sub y2 y1 sub Pyth def
				/dArrowPos \psk@ArrowInsidePos\space abs def
				{
					/ArrowPos ArrowPos dArrowPos add def
					ArrowPos Length gt { exit } if
					x1 Alpha cos ArrowPos mul add
					y1 Alpha sin ArrowPos mul add
					ArrowInside
					pop pop
				} loop
			}{
				/ArrowPos \psk@ArrowInsideOffset\space def
				/dArrowPos \psk@ArrowInsideNo 1 gt {%
					1.0 \psk@ArrowInsideNo 1.0 add div
				}{ \psk@ArrowInsidePos } ifelse def
				\psk@ArrowInsideNo\space cvi {
					/ArrowPos ArrowPos dArrowPos add def
					x2 x1 sub ArrowPos mul x1 add
					y2 y1 sub ArrowPos mul y1 add
					ArrowInside
					pop pop
				} repeat
			} ifelse
			pop pop Lineto
		} repeat
	}{ ArrowA /n n 2 sub def n { Lineto } repeat } ifelse
	CP 4 2 roll ArrowB L pop pop } if%
}>
%
% Redefinition of the PostScript /Polygon macro to print the intermediate
% arrow on each segment of the line
\pst@def{Polygon}<{%
	NArray n 2 eq { 0 0 /n 3 def } if
	n 3 lt {
		n { pop pop } repeat
	}{
		n 3 gt { CheckClosed } if
		n 2 mul
		-2 roll
		/y0 ED
    	/x0 ED
    	/y1 ED
    	/x1 ED
    	/xx1 x1 def
    	/yy1 y1 def
    	x1 y1
    	/x1 x0 x1 add 2 div def
    	/y1 y0 y1 add 2 div def
    	x1 y1 moveto
    	/n n 2 sub def
		/drawArrows {
			x11 y11
			\psk@ArrowInsidePos\space 1 gt {
				/Alpha y12 y11 sub x12 x11 sub atan def
				/ArrowPos \psk@ArrowInsideOffset\space def
				/Length x12 x11 sub y12 y11 sub Pyth def
				/dArrowPos \psk@ArrowInsidePos\space abs def
				{
					/ArrowPos ArrowPos dArrowPos add def
					ArrowPos Length gt { exit } if
					x11 Alpha cos ArrowPos mul add
					y11 Alpha sin ArrowPos mul add
					ArrowInside
					pop pop
				} loop
			}{
				/ArrowPos \psk@ArrowInsideOffset\space def
				/dArrowPos \psk@ArrowInsideNo 1 gt {%
					1.0 \psk@ArrowInsideNo 1.0 add div
				}{ \psk@ArrowInsidePos } ifelse def
					\psk@ArrowInsideNo cvi {
					/ArrowPos ArrowPos dArrowPos add def
					x12 x11 sub ArrowPos mul x11 add
					y12 y11 sub ArrowPos mul y11 add
        			ArrowInside
					pop pop
				} repeat
			} ifelse
			pop pop Lineto
		} def
		n {
			4 copy
			/y11 ED /x11 ED /y12 ED /x12 ED
			drawArrows
		} repeat
		x1 y1 x0 y0
		6 4 roll
		2 copy
		/y11 ED /x11 ED /y12 y0 def /x12 x0 def
		drawArrows
		/y11 y0 def /x11 x0 def /y12 yy1 def /x12 xx1 def
		drawArrows
		pop pop
    	closepath
	} ifelse %
}>
%
%
% Redefinition of the PostScript /OpenBezier macro to print the intermediate
% arrow
\pst@def{OpenBezier}<{%
	/dArrowPos \psk@ArrowInsideNo 1 gt {%
		1.0 \psk@ArrowInsideNo 1.0 add div
	}{ \psk@ArrowInsidePos } ifelse def
	BezierNArray
	n 1 eq { pop pop
	}{ 2 copy
		/y0 ED /x0 ED
		ArrowA
		n 4 sub 3 idiv { 6 2 roll 4 2 roll curveto } repeat
		6 2 roll
		4 2 roll
		ArrowB
		/y3 ED /x3 ED /y2 ED /x2 ED /y1 ED /x1 ED
    	/cx x1 x0 sub 3 mul def
		/cy y1 y0 sub 3 mul def
		/bx x2 x1 sub 3 mul cx sub def
		/by y2 y1 sub 3 mul cy sub def
		/ax x3 x0 sub cx sub bx sub def
		/ay y3 y0 sub cy sub by sub def
		/getValues {
			ax t0 3 exp mul bx t0 t0 mul mul add cx t0 mul add x0 add
			ay t0 3 exp mul by t0 t0 mul mul add cy t0 mul add y0 add
			ax t 3 exp mul bx t t mul mul add cx t mul add x0 add
			ay t 3 exp mul by t t mul mul add cy t mul add y0 add
		} def
		/getdL {
			getValues
			3 -1 roll sub 3 1 roll sub Pyth
		} def
		/CurveLength {
			/u 0 def
			/du 0.01 def
			0 100 {
				/t0 u def
				/u u du add def
				/t u def
				getdL add
			} repeat } def
		/GetArrowPos {
			/ende \psk@ArrowInsidePos\space 1 gt
				{ArrowPos}
				{ArrowPos CurveLength mul} ifelse def
			/u 0 def
			/du 0.01 def
			/sum 0 def
			{
				/t0 u def
				/u u du add def
		    	/t u def
				/sum getdL sum add def
				sum ende gt {exit} if
			} loop u
		} def
		/ArrowPos \psk@ArrowInsideOffset\space def
		/loopNo \psk@ArrowInsidePos\space 1 gt {%
			CurveLength \psk@ArrowInsidePos\space div cvi
			}{ \psk@ArrowInsideNo } ifelse def
		loopNo cvi {
			/ArrowPos ArrowPos dArrowPos add def
			/t GetArrowPos def
			/t0 t 0.95 mul def
			getValues
			ArrowInside pop pop pop pop
		} repeat
		x1 y1 x2 y2 x3 y3 curveto
	} ifelse
}>
%
% Redefinition of the PostScript /NCLine macro to print the intermediate
% arrow of the line
\pst@def{NCLine}<{%
	NCCoor
	tx@Dict begin
	ArrowA CP 4 2 roll ArrowB
	4 copy
	/y2 ED /x2 ED /y1 ED /x1 ED
	x1 y1
	\psk@ArrowInsidePos\space 1 gt{
		/Alpha y2 y1 sub x2 x1 sub atan def
		/ArrowPos \psk@ArrowInsideOffset\space def
		/Length x2 x1 sub y2 y1 sub Pyth def
		/dArrowPos \psk@ArrowInsidePos\space abs def
		{
			/ArrowPos ArrowPos dArrowPos add def
			ArrowPos Length gt { exit } if
			x1 Alpha cos ArrowPos mul add
			y1 Alpha sin ArrowPos mul add
			ArrowInside
			pop pop
		} loop
	}{
		/ArrowPos \psk@ArrowInsideOffset\space def
		/dArrowPos \psk@ArrowInsideNo 1 gt {%
			1.0 \psk@ArrowInsideNo 1.0 add div
		}{ \psk@ArrowInsidePos } ifelse def
		\psk@ArrowInsideNo\space cvi {
			/ArrowPos ArrowPos dArrowPos add def
			x2 x1 sub ArrowPos mul x1 add
			y2 y1 sub ArrowPos mul y1 add
			ArrowInside
			pop pop
		} repeat
	} ifelse
	pop pop lineto pop pop
	end%
}>
%
\pst@def{NCCurve}<{%
	GetEdgeA GetEdgeB
	xA1 xB1 sub yA1 yB1 sub
	Pyth 2 div dup 3 -1 roll mul
	/ArmA ED
	mul
	/ArmB ED
	/ArmTypeA 0 def
	/ArmTypeB 0 def
	GetArmA GetArmB
	xA2 yA2 xA1 yA1
	2 copy
	/y0 ED /x0 ED
	tx@Dict begin
		ArrowA
	end
	xB2 yB2 xB1 yB1
	tx@Dict begin
		ArrowB
	end
	/y3 ED /x3 ED /y2 ED /x2 ED /y1 ED /x1 ED
	/cx x1 x0 sub 3 mul def
	/cy y1 y0 sub 3 mul def
	/bx x2 x1 sub 3 mul cx sub def
	/by y2 y1 sub 3 mul cy sub def
	/ax x3 x0 sub cx sub bx sub def
	/ay y3 y0 sub cy sub by sub def
	/getValues {
		ax t0 3 exp mul bx t0 t0 mul mul add cx t0 mul add x0 add
		ay t0 3 exp mul by t0 t0 mul mul add cy t0 mul add y0 add
		ax t 3 exp mul bx t t mul mul add cx t mul add x0 add
	ay t 3 exp mul by t t mul mul add cy t mul add y0 add
	} def
	/getdL {
		getValues
		3 -1 roll sub 3 1 roll sub Pyth
	} def
	/CurveLength {
		/u 0 def
		/du 0.01 def
		0 100 {
			/t0 u def
			/u u du add def
			/t u def
			getdL add
		} repeat } def
	/GetArrowPos {
		/ende \psk@ArrowInsidePos\space 1 gt {ArrowPos}{ArrowPos CurveLength mul} ifelse def
		/u 0 def
		/du 0.01 def
		/sum 0 def
		{
			/t0 u def
			/u u du add def
			/t u def
			/sum getdL sum add def
			sum ende gt {exit} if
		} loop u
	} def
	/dArrowPos \psk@ArrowInsideNo 1 gt {%
		1.0 \psk@ArrowInsideNo 1.0 add div
	}{ \psk@ArrowInsidePos } ifelse def
	/ArrowPos \psk@ArrowInsideOffset\space def
	/loopNo \psk@ArrowInsidePos\space 1 gt {%
		CurveLength \psk@ArrowInsidePos\space div cvi
		}{ \psk@ArrowInsideNo } ifelse def
	loopNo cvi {
		/ArrowPos ArrowPos dArrowPos add def
		/t GetArrowPos def
		/t0 t 0.95 mul def
		getValues
		ArrowInside pop pop pop pop
	} repeat
	x1 y1 x2 y2 x3 y3 curveto
	/LPutVar [ xA1 yA1 xA2 yA2 xB2 yB2 xB1 yB1 ] cvx def
	/LPutPos { t LPutVar BezierMidpoint } def
	/HPutPos { { HPutLines } HPutCurve } def
	/VPutPos { { VPutLines } HPutCurve } def
}>
%
\def\psset@dashColorI#1{\pst@getcolor{#1}\psDashColorI}
\def\psset@dashColorII#1{\pst@getcolor{#1}\psDashColorII}
\define@key{psset}{dashNo}{\edef\psk@dashNo{#1}}
%
\define@key{psset}{linecap}{\edef\psk@linecap{#1}}
\psset{dashColorI=black,dashColorII=red,dashNo=0.2,linecap=0}
%
\pst@def{LineII}<{%
	NArray
	/n n 1 sub def
	/y1 ED /x1 ED x1 y1 ArrowA x1 y1 moveto
	\psk@linecap\space 3 gt
		{\psk@linecap\space 0 lt {0 setlinecap} if }
		{\psk@linecap\space setlinecap} ifelse
	n {
		/y2 ED /x2 ED
		/y0 y1 def /x0 x1 def
		/length x2 x1 sub y2 y1 sub Pyth def
		\psk@dashNo\space 1.0 lt
			{/cntMax 1.0 \psk@dashNo\space div .49 add cvi def}
			{/cntMax length \psk@dashNo\space div .49 add cvi def} ifelse
		x2 x1 sub cntMax div /dx ED
		y2 y1 sub cntMax div /dy ED
		/cnt 0 def
		cntMax {
			gsave
			/x1 x1 dx add def
			/y1 y1 dy add def
			x1 y1
			cnt 2 mod 0 eq
				{ \pst@usecolor\psDashColorI }
				{ \pst@usecolor\psDashColorII } ifelse
			lineto stroke
			/cnt cnt 1 add def
			grestore
			x1 y1 moveto
		} repeat
		/y1 y2 def /x1 x2 def
	} repeat
	x0 y0 x2 y2 ArrowB L pop pop
}>
%
\def\pslineII{\pst@object{pslineII}}
\def\pslineII@i{%
    \pst@getarrows{%
        \begin@OpenObj
        \pst@getcoors[\pslineII@ii%
    }%
}
\def\pslineII@ii{%
	\addto@pscode{%
		\pst@cp
		\ifshowpoints true \else false \fi
		\tx@LineII
	}%
	\end@OpenObj%
}
%
\newdimen\pswBegin\newdimen\pswEnd
\def\psset@wBegin#1{\pssetlength\pswBegin{#1}}
\def\psset@wEnd#1{\pssetlength\pswEnd{#1}}
\setkeys{psset}{wBegin=\pslinewidth, wEnd=\pslinewidth}
%
\pst@def{LineIII}<{%
	NArray
	/n n 1 sub def
	/YA ED /XA ED
	/bA2 \pst@number\pswBegin\space 2.0 div def
	/bB2 \pst@number\pswEnd\space 2.0 div def
	/xStep bB2 bA2 sub n div def
	0 setlinecap
	n {
		XA YA moveto
		/YB ED /XB ED
		/Alpha YB YA sub XB XA sub atan def
		/Alphasin Alpha sin def
		/Alphacos Alpha cos def
        \pst@usecolor\pslinecolor
		0.01 SLW
		/bB2 bA2 xStep add def
		XA Alphasin bA2 mul sub
		YA Alphacos bA2 mul add lineto
		XB Alphasin bB2 mul sub
		YB Alphacos bB2 mul add lineto
		XB Alphasin bB2 mul add
		YB Alphacos bB2 mul sub lineto
		XA Alphasin bA2 mul add
		YA Alphacos bA2 mul sub lineto
		XA YA lineto fill
		/XA XB def /YA YB def
		/bA2 bB2 def
	} repeat
}>
%
\def\pslineIII{\pst@object{pslineIII}}
\def\pslineIII@i{%
    \pst@getarrows{%
        \begin@OpenObj
        \pst@getcoors[\pslineIII@ii%
    }%
}
\def\pslineIII@ii{%
	\addto@pscode{%
		\pst@cp
		\ifshowpoints true \else false \fi
		\tx@LineIII
	}%
	\end@OpenObj%
}
%
\catcode`\@=\PstAtCode\relax
%
%% END: pstricks-add.tex
\endinput

%% CHANGE-LOG
% v 0.9c	add \psFormatInt
% v 0.9b	add \pslineIII
% v 0.9a	add relative dashNo
% v 0.9		add \pslineII
% v 0.8e	add bracePos
% v 0.8d	fix bug in arrows
% v 0.8c	small tweaks to \@@rput@iv
% v 0.8b	now every object can be passed to psbrace
% v 0.8a	fix bug with arrow
% v 0.8		ArrowFill added
% v 0.7a	adding option asolid as fillstyle
% v 0.7		ArrowInsidePos>1 for all macros
% v 0.6		ArrowInsidePos>1 sets nowthe arrows every n-th pt
% v 0.5a	small improvements to the code (use of Pyth)
% v 0.5		new psbezier and pcline to get the arrows in the right place!
% v 0.4		fix bug in psbezier and nccurve, to get the right arrow position

